Coronal magnetic field and emission properties of small-scale bright and faint loops in the quiet Sun

The present study provides statistical information on the coronal magnetic field and intensity properties of small-scale bright and faint loops in the quiet Sun. We aim to quantitatively investigate the morphological and topological properties of the coronal magnetic field in bright and faint small-scale loops, with the former known as coronal bright points (CBPs). We analyse 126 small-scale loops using quasi-temporal imaging and line-of-sight magnetic field observations. We employ a recently developed automatic tool that uses a linear magneto-hydro-static model to compute the magnetic field in the solar atmosphere and automatically match individual magnetic field lines with small-scale loops. For most of the loops, we automatically obtain an excellent agreement of the magnetic field lines from the LMHS model and the loops seen in AIA 193 A. One stand-out result is that the magnetic field is non-potential. We obtain the typical ranges of loop heights, lengths, intensities, mean magnetic field strength along the loops and at loop tops, and magnetic field strength at loop footpoints. We find that loops below the classic chromospheric height of 1.5 Mm are flatter suggesting that non-magnetic forces (one of which is the plasma pressure) play an important role below this height. We find a strong correlation (Pearson coefficient of 0.9) between loop heights and lengths. The average intensity along the loops correlates stronger with the average magnetic field along the loops than with the field strength at loop tops. The latter correlation indicates that the energy release in the loops is more likely linked to the average magnetic field along the loops than the field strength on the loop tops. In other words, the energy is probably released all along the loops, but not just at the loop top. This result is consistent with the recent benchmarking radiative 3D MHD model of N\'obrega-Siberio etal.

==> figures/table2b.tex <==
\onecolumn
\begin{center}
\begin{longtable}{|l|l|l|l|l|l|l|l|l|l|l|}
\caption{Coronal magnetic properties of small-scale loops in the quiet Sun.}
 \hline\multicolumn{1}{|c}{Case}&\multicolumn{1}{|c}{L$_{MHS}$}& \multicolumn{1}{|c}{$\alpha$}&\multicolumn{1}{|c}{$a$}&\multicolumn{1}{|c}{$\kappa$}&\multicolumn{1}{|c}{Par}&\multicolumn{1}{|c}{Bright}&\multicolumn{1}{|c}{L [Mm]}&\multicolumn{1}{|c}{H[Mm]}&\multicolumn{1}{|c}{Bpos}&\multicolumn{1}{|c|}{Bneg}
\endfirsthead
 \multicolumn{11}{c} {{ \tablename\ \thetable{} -- Continued from previous page}} \\
 \hline
\multicolumn{1}{|c}{Case}&\multicolumn{1}{|c}{L$_{MHS}$}& \multicolumn{1}{|c}{$\alpha$}&\multicolumn{1}{|c}{$a$}&\multicolumn{1}{|c}{$\kappa$} & \multicolumn{1}{|c}{Par}&\multicolumn{1}{|c}{Bright}&
\multicolumn{1}{|c}{L [Mm]}&\multicolumn{1}{|c}{H[Mm]}&\multicolumn{1}{|c}{Bpos}&\multicolumn{1}{|c|}{Bneg}
 \\ \hline
\endhead
\hline
\multicolumn{11}{c}{Continued on next page}
\endfoot
 \endlastfoot
 \hline
001 bp001\_fr\_111 &   0.49& -0.62 &  0.43 &  0.73&  St &   84.27 &  13.992 &   1.389 &    16.4 &   -11.3\\
006 bp002\_fr\_095 &   0.01&  0.01 &  1.00 &  0.73&  St &  111.77 &   3.307 &   0.344 &    17.5 &   -10.7\\
007 bp002\_fr\_134 &   0.01& -0.35 &  0.89 &  0.30&  St &  117.85 &   4.816 &   0.188 &    11.5 &    -5.7\\
011 bp004\_fr\_000 &   0.28& -2.41 &  0.43 &  0.77&  NSt &   67.40 &  17.966 &   6.110 &    62.4 &  -189.5\\
012 bp006\_fr\_025 &   0.30&  0.99 &  0.68 &  0.69&  St &  126.18 &  16.410 &   3.875 &    18.0 &  -228.1\\
013 bp006\_fr\_059 &   0.02&  5.98 &  0.71 &  0.46&  NSt &  204.65 &   8.237 &   1.520 &    22.2 &  -139.6\\
018 bp007\_fr\_046 &   0.05&  3.12 &  0.81 &  0.59&  NSt &  258.77 &  18.600 &   5.981 &    78.0 &  -119.8\\
019 bp007\_fr\_070 &   0.00& -2.02 &  0.45 &  0.98&  NSt &  221.98 &  11.459 &   2.725 &    42.5 &   -52.2\\
020 bp007\_fr\_103 &   1.20&  0.75 &  0.58 &  0.48&  St &  205.33 &  20.576 &   4.933 &     4.3 &  -237.8\\
022 bp008\_fr\_021 &   0.16& -2.72 &  0.00 &  0.00&  NSt &  173.11 &   6.554 &   1.166 &    85.6 &   -32.9\\
023 bp008\_fr\_042 &   0.05& -2.24 &  0.60 &  0.60&  St &  220.93 &   8.483 &   1.278 &     3.0 &   -19.9\\
024 bp008\_fr\_056 &   0.39& -0.58 &  0.67 &  0.32&  St &  254.35 &  13.554 &   3.046 &    64.7 &    -2.3\\
027 bp009\_fr\_111 &   0.13& -2.11 &  0.82 &  0.71&  St &  160.40 &  24.486 &   7.773 &   197.8 &   -83.8\\
028 bp009\_fr\_146 &   0.01&  3.92 &  0.47 &  0.97&  NSt &  175.05 &  14.498 &   4.016 &   108.2 &   -57.7\\
030 bp014\_fr\_075 &   0.06&  0.27 &  0.77 &  0.26&  St &  321.37 &   7.163 &   1.091 &    51.6 &   -16.0\\
031 bp014\_fr\_084 &   1.13&  1.21 &  0.29 &  0.53&  St &  338.64 &  13.834 &   0.937 &    70.7 &   -77.9\\
032 bp014\_fr\_095 &   0.80& -2.58 &  1.00 &  0.87&  St &  320.79 &  16.488 &   1.593 &    15.5 &   -80.7\\
034 bp015\_fr\_016 &   0.07&  1.83 &  0.71 &  0.35&  St &  130.51 &  10.778 &   2.747 &    71.0 &   -74.7\\
037 bp015\_fr\_179 &   0.01& -0.78 &  0.82 &  0.30&  NSt &  204.05 &   6.321 &   1.021 &     5.1 &  -114.3\\
039 bp016\_fr\_070 &   0.08& -0.14 &  0.00 &  0.00&  NSt &  106.73 &   9.766 &   2.081 &    43.2 &  -145.8\\
040 bp016\_fr\_090 &   0.03& -5.15 &  1.00 &  0.41&  NSt &   87.16 &   5.548 &   1.002 &    12.1 &   -26.0\\
041 bp016\_fr\_128 &   0.01&  2.21 &  0.97 &  0.62&  NSt &  107.16 &   6.514 &   1.214 &    22.4 &   -26.5\\
042 bp016\_fr\_133 &   0.01&  2.24 &  1.00 &  0.46&  NSt &  120.75 &   6.389 &   1.015 &    25.5 &   -61.1\\
043 bp017\_fr\_027 &   2.09&  1.54 &  0.77 &  0.53&  St &  121.98 &  13.205 &   2.065 &    51.7 &   -51.7\\
044 bp019\_fr\_177 &   0.01& -0.16 &  0.89 &  0.53&  St &  357.31 &   9.685 &   0.866 &    44.7 &   -33.9\\
045 bp019\_fr\_178 &   0.00&  0.16 &  1.00 &  0.56&  St &  385.28 &   9.907 &   0.855 &    47.4 &   -47.4\\
046 bp019\_fr\_229 &   1.89& -4.74 &  0.71 &  0.68&  St &  101.77 &  23.844 &   6.889 &   176.1 &   -66.4\\
048 bp019\_fr\_272 &   0.00& -3.48 &  0.00 &  0.00&  St &  292.25 &   1.353 &   0.012 &    12.4 &   -12.4\\
049 bp019\_fr\_326 &   0.03& -5.47 &  0.88 &  0.63&  St &   89.50 &   7.473 &   1.023 &    29.7 &    -1.1\\
051 bp021\_fr\_143 &   1.86& -0.47 &  0.94 &  0.16&  St &   95.79 &  11.175 &   0.754 &    14.4 &   -10.5\\
052 bp021\_fr\_154 &   0.98& -0.87 &  0.48 &  0.49&  St &  112.90 &  26.812 &   9.331 &   144.4 &   -64.2\\
053 bp022\_fr\_000 &   0.11&  1.81 &  0.59 &  0.31&  St &   67.40 &  16.956 &   2.630 &    97.0 &   -16.7\\
054 bp022\_fr\_032 &   0.05&  4.63 &  0.63 &  0.86&  NSt &  131.72 &   8.437 &   1.387 &    75.5 &   -60.9\\
056 bp022\_fr\_244 &   0.78&  5.76 &  0.97 &  0.37&  St &  118.86 &  15.991 &   2.015 &    23.9 &    -5.6\\
057 bp022\_fr\_255 &   0.60&  5.72 &  0.30 &  0.89&  St &  109.73 &  21.571 &   4.443 &    12.1 &  -170.6\\
058 bp022\_fr\_273 &   0.02&  2.54 &  0.95 &  0.63&  St &  237.57 &  19.450 &   5.497 &    26.9 &  -302.0\\
059 bp023\_fr\_028 &   0.02& -0.93 &  0.84 &  0.39&  NSt &  161.99 &  12.550 &   2.686 &    10.6 &  -162.5\\
060 bp023\_fr\_113 &   0.21& -0.29 &  0.72 &  0.48&  NSt &   80.95 &  17.463 &   3.401 &   105.8 &   -10.0\\
062 bp023\_fr\_115 &  30.24& -3.13 &  0.00 &  0.00&  St &   78.05 &  19.049 &   2.371 &    10.7 &   -34.6\\
063 bp023\_fr\_171 &   0.24& -2.90 &  0.23 &  0.71&  St &  115.64 &   8.348 &   1.289 &    20.1 &    -9.7\\
064 bp023\_fr\_217 &   0.14& -3.41 &  1.00 &  0.49&  St &  236.51 &   6.458 &   1.177 &     5.2 &  -109.7\\
065 bp024\_fr\_052 &  15.75&  3.92 &  0.00 &  0.00&  St &  241.47 &  33.366 &   8.571 &    95.5 &  -503.5\\
067 bp026\_fr\_011 &   0.08&  4.54 &  0.99 &  0.73&  St &   63.19 &   9.031 &   1.538 &    32.0 &    -1.4\\
068 bp026\_fr\_013 &   0.10&  3.44 &  0.12 &  0.81&  St &   75.89 &  10.670 &   1.199 &    35.5 &   -14.1\\
069 bp026\_fr\_014 &   0.19& -0.51 &  1.00 &  0.30&  St &   75.09 &  13.582 &   3.851 &   114.8 &   -82.9\\
070 bp026\_fr\_020 &   0.13&  4.35 &  1.00 &  0.70&  St &  207.91 &  10.217 &   1.436 &    79.0 &   -13.8\\
071 bp026\_fr\_021 &   0.09& -2.61 &  1.00 &  0.38&  St &  224.34 &  17.488 &   5.281 &   190.8 &  -219.9\\
072 bp026\_fr\_136 &   2.21&  0.29 &  0.38 &  0.45&  NSt &  137.97 &  17.870 &   5.297 &   108.5 &   -27.7\\
073 bp026\_fr\_155 &   0.05&  5.87 &  0.95 &  0.62&  St &  334.52 &  16.409 &   4.602 &   111.3 &  -103.2\\
074 bp026\_fr\_156 &   0.11&  3.90 &  0.00 &  0.00&  St &  180.61 &   8.269 &   0.703 &     5.9 &   -30.4\\
075 bp026\_fr\_157 &   0.07&  4.32 &  0.97 &  0.34&  St &  276.95 &  10.110 &   2.601 &   146.4 &  -135.5\\
076 bp026\_fr\_159 &   0.21&  3.13 &  0.53 &  0.64&  St &  302.36 &  16.790 &   5.275 &    53.1 &   -48.6\\
077 bp026\_fr\_160 &   0.34&  3.86 &  0.48 &  0.55&  St &  272.03 &  18.112 &   5.631 &    47.0 &   -43.4\\
078 bp026\_fr\_161 &   1.30&  2.79 &  0.57 &  0.18&  St &  237.52 &  22.683 &   7.174 &    43.5 &   -92.9\\
079 bp026\_fr\_199 &   0.06&  3.54 &  0.61 &  1.00&  St &  430.95 &  21.413 &   6.333 &    96.9 &  -106.6\\
081 bp026\_fr\_202 &   0.82&  6.00 &  0.96 &  0.57&  St &  322.40 &  17.574 &   3.406 &   313.0 &   -95.2\\
082 bp026\_fr\_260 &   1.17&  1.29 &  0.88 &  1.00&  NSt &  251.88 &  15.713 &   3.034 &    49.0 &   -63.6\\
083 bp026\_fr\_263 &  11.73&  1.86 &  0.16 &  0.26&  St &  127.72 &  26.908 &   4.346 &   173.4 &   -85.8\\
084 bp026\_fr\_273 &   0.07&  2.41 &  1.00 &  0.69&  NSt &  307.96 &  24.019 &   6.696 &   129.6 &  -156.5\\
085 bp028\_fr\_026 &   0.43&  2.84 &  0.00 &  0.00&  St &  286.70 &  12.809 &   1.171 &    88.9 &   -22.3\\
086 bp028\_fr\_029 &   0.54&  1.24 &  0.11 &  0.60&  St &  345.65 &  21.672 &   6.421 &   259.2 &  -104.7\\
087 bp028\_fr\_033 &   0.04&  1.22 &  1.00 &  0.74&  St &  380.68 &  13.188 &   1.422 &   112.9 &   -73.3\\
088 bp028\_fr\_034 &   0.75&  1.96 &  1.00 &  0.30&  St &  359.46 &  15.122 &   1.768 &   117.9 &   -81.7\\
089 bp028\_fr\_092 &   0.38&  3.60 &  0.89 &  0.62&  St &  486.81 &  12.684 &   1.398 &    25.6 &   -27.9\\
090 bp028\_fr\_169 &   0.12&  5.94 &  0.51 &  0.51&  St &  431.07 &  12.411 &   1.535 &     6.2 &   -17.0\\
091 bp028\_fr\_197 &   0.79&  4.05 &  0.59 &  0.57&  St &  453.16 &  18.611 &   4.275 &   214.2 &   -93.2\\
094 bp029\_fr\_181 &  38.76& -2.66 &  0.69 &  0.62&  St &   91.62 &  45.195 &  13.001 &   129.0 &  -130.5\\
095 bp029\_fr\_187 &  58.95& -3.06 &  0.26 &  0.54&  NSt &  101.60 &  35.794 &   6.995 &   240.3 &   -19.5\\
096 bp029\_fr\_190 &  66.15& -2.31 &  0.68 &  0.63&  St &  100.92 &  35.920 &   7.801 &    39.8 &   -76.6\\
097 bp029\_fr\_202 &  98.95& -3.01 &  0.67 &  0.60&  St &  107.81 &  30.813 &   4.652 &    33.0 &   -16.2\\
100 bp029\_fr\_224 &  23.37& -3.13 &  1.00 &  0.50&  St &  104.89 &  44.807 &  12.593 &   140.5 &  -135.5\\
101 bp029\_fr\_227 &   0.26& -2.88 &  0.00 &  0.00&  St &  133.17 &  31.233 &   5.629 &    23.2 &   -91.3\\
102 bp029\_fr\_228 &   1.60& -2.78 &  0.19 &  0.21&  St &  131.41 &  25.895 &   1.907 &    23.9 &   -27.6\\
104 bp029\_fr\_332 &   0.80& -2.21 &  0.69 &  0.61&  NSt &  160.36 &  32.004 &   8.020 &    46.5 &    -5.0\\
105 bp029\_fr\_375 &   0.50&  0.05 &  1.00 &  0.99&  St &  140.40 &  40.513 &  11.987 &   244.1 &  -359.3\\
106 bp031\_fr\_143 &   0.75&  2.18 &  0.99 &  0.51&  St &  106.08 &  12.929 &   1.575 &     4.1 &   -94.0\\
107 bp031\_fr\_170 &   0.05& -0.02 &  0.97 &  0.05&  St &  142.40 &   8.294 &   1.637 &     4.0 &   -12.1\\
110 bp033\_fr\_031 &   0.06&  4.36 &  0.94 &  0.83&  St &  106.17 &   7.135 &   1.250 &     3.5 &    -2.1\\
111 bp033\_fr\_091 &   0.05&  3.45 &  0.00 &  0.00&  St &  114.43 &  11.368 &   0.535 &    39.4 &   -12.4\\
112 bp033\_fr\_252 &   0.00&  1.93 &  0.65 &  0.47&  St &  188.58 &   7.054 &   1.168 &    69.6 &   -13.8\\
113 bp033\_fr\_264 &   0.00&  1.45 &  0.67 &  0.63&  St &  138.29 &   5.199 &   0.706 &    13.2 &   -19.9\\
115 bp035\_fr\_039 &   0.61& -4.88 &  0.00 &  0.00&  NSt &  173.92 &  17.104 &   4.769 &   197.7 &   -27.9\\
117 bp035\_fr\_115 &   0.04&  1.75 &  1.00 &  0.66&  St &  144.26 &   8.992 &   1.217 &    25.9 &  -147.4\\
119 bp038\_fr\_355 &  10.33& -5.64 &  0.00 &  0.00&  NSt &   69.08 &  17.362 &   1.534 &    64.9 &    -0.3\\
121 bp040\_fr\_157 & 278.88&  1.18 &  0.00 &  0.00&  St &   58.74 &  60.543 &  12.740 &    68.8 &    -8.9\\
128 bp044\_fr\_122 &   0.05& -1.03 &  0.90 &  0.73&  NSt &  104.33 &   6.275 &   1.642 &    55.9 &  -111.6\\
131 bp048\_fr\_424 &  99.53& -2.53 &  0.63 &  0.74&  St &   75.00 &  40.075 &   9.854 &    60.2 &   -13.2\\
132 bp050\_fr\_012 &  59.60& -3.22 &  0.47 &  0.69&  St &   94.50 &  24.130 &   6.990 &    72.8 &  -116.5\\
133 bp050\_fr\_102 &   3.70& -2.16 &  0.45 &  0.53&  St &  111.98 &  23.902 &   6.203 &    25.8 &  -150.2\\
134 bp050\_fr\_110 &   0.69& -0.80 &  0.36 &  0.35&  St &  116.06 &  17.605 &   3.610 &     3.8 &   -69.9\\
135 bp050\_fr\_146 &   0.03&  2.39 &  0.49 &  0.91&  NSt &  161.49 &  21.680 &   6.212 &    43.1 &   -86.8\\
136 bp050\_fr\_203 &   0.34&  2.16 &  0.99 &  1.00&  St &  124.74 &  16.799 &   3.010 &    95.9 &   -93.4\\
137 bp050\_fr\_212 &   0.20&  0.07 &  1.00 &  0.00&  St &  129.40 &  14.909 &   3.124 &    91.8 &   -80.5\\
138 bp050\_fr\_262 &  25.29& -0.09 &  0.98 &  0.81&  St &  102.44 &  30.827 &  11.347 &   218.5 &   -26.9\\
139 bp055\_fr\_015 &   0.20&  0.47 &  1.00 &  0.65&  St &   74.80 &  15.954 &   4.980 &   164.2 &  -184.8\\
141 bp055\_fr\_022 &   0.08& -1.69 &  1.00 &  0.66&  St &  224.92 &  16.592 &   4.777 &   234.1 &  -202.6\\
142 bp055\_fr\_027 &   0.02&  0.11 &  1.00 &  0.54&  St &  359.49 &  10.728 &   1.987 &   169.6 &   -27.8\\
144 bp055\_fr\_038 &   0.07& -0.50 &  0.65 &  0.60&  St &  315.41 &  14.609 &   3.235 &   119.7 &   -69.8\\
145 bp056\_fr\_036 &   0.45& -2.61 &  0.11 &  0.57&  St &  152.95 &  20.535 &   4.525 &     3.1 &  -121.1\\
152 bp058\_fr\_067 &   0.07&  2.03 &  0.22 &  0.07&  NSt &  237.77 &   8.353 &   2.329 &    99.1 &  -140.8\\
153 bp061\_fr\_012 &   0.29&  1.84 &  0.14 &  0.76&  St &  195.45 &   9.828 &   1.589 &    90.2 &   -50.1\\
154 bp061\_fr\_018 &   0.05&  1.73 &  0.87 &  0.95&  St &  182.54 &   8.385 &   0.507 &    24.8 &   -22.8\\
156 bp061\_fr\_163 &   0.02&  4.82 &  1.00 &  0.63&  St &  125.85 &   4.181 &   0.567 &    46.1 &   -10.6\\
157 bp062\_fr\_073 &   7.20& -1.26 &  1.00 &  0.11&  NSt &  133.19 &  35.223 &  13.330 &   116.7 &   -72.4\\
158 bp062\_fr\_088 &  58.34& -0.87 &  0.88 &  0.71&  St &   94.68 &  20.353 &   2.527 &     9.2 &   -14.2\\
159 bp062\_fr\_157 &   0.56&  1.86 &  0.98 &  0.22&  St &  229.14 &  19.119 &   6.897 &   194.1 &   -47.3\\
160 bp062\_fr\_159 &   0.20& -0.73 &  1.00 &  0.26&  St &  237.12 &  20.014 &   7.287 &   219.8 &   -43.8\\
161 bp062\_fr\_160 &   0.01& -3.27 &  0.57 &  0.24&  NSt &  303.99 &   6.993 &   1.890 &   172.8 &   -55.4\\
162 bp065\_fr\_094 &   0.15&  2.97 &  0.51 &  1.00&  NSt &  101.30 &  18.879 &   5.139 &   157.6 &   -38.4\\
164 bp066\_fr\_038 &  15.93&  0.11 &  0.29 &  0.81&  St &  218.97 &  27.307 &   7.643 &   199.5 &   -95.7\\
166 bp066\_fr\_040 &   0.00& -0.52 &  0.29 &  0.56&  St &  204.21 &   4.970 &   0.585 &    21.6 &   -22.2\\
167 bp066\_fr\_052 &   0.93& -0.55 &  0.89 &  0.29&  St &  268.37 &  11.235 &   3.176 &   105.3 &   -72.0\\
168 bp066\_fr\_056 &   1.74&  5.45 &  0.53 &  0.74&  St &  320.41 &  10.549 &   2.071 &    41.2 &   -10.9\\
170 bp066\_fr\_066 &   0.03& -0.82 &  1.00 &  0.29&  NSt &  593.21 &  13.530 &   3.495 &   273.3 &  -175.8\\
171 bp066\_fr\_205 &   1.36&  2.58 &  0.31 &  0.38&  St &  518.21 &  30.050 &   9.785 &   341.5 &  -176.9\\
174 bp075\_fr\_000 &  45.95& -5.62 &  0.46 &  0.49&  St &   81.71 &  27.782 &   2.048 &    37.4 &   -53.9\\
176 bp075\_fr\_025 &  22.73& -4.20 &  0.67 &  0.37&  St &   66.42 &  39.769 &  12.510 &   119.2 &   -80.8\\
177 bp075\_fr\_216 &   0.23&  0.42 &  0.80 &  0.78&  St &   69.33 &  11.259 &   0.989 &    50.2 &   -15.9\\
178 bp086\_fr\_022 &   0.02& -2.78 &  0.85 &  0.94&  St &  170.43 &   8.678 &   0.961 &    89.8 &   -52.4\\
180 bp086\_fr\_025 &   0.00& -1.46 &  0.00 &  0.00&  St &  343.67 &   7.933 &   2.015 &   394.3 &   -58.4\\
181 bp092\_fr\_094 &  26.30& -2.16 &  0.40 &  0.79&  St &   72.70 &  35.085 &  11.235 &   210.7 &  -104.8\\
184 bp111\_fr\_006 &   0.78&  1.68 &  0.00 &  0.00&  St &   91.57 &  11.762 &   1.238 &    22.8 &    -5.1\\
185 bp111\_fr\_029 &   0.26&  5.91 &  0.93 &  0.57&  St &   72.43 &   3.872 &   0.351 &     7.6 &    -0.9\\
187 bp111\_fr\_040 &   0.04&  4.77 &  0.88 &  0.57&  St &  118.08 &   8.297 &   2.204 &   103.3 &   -29.4\\
188 bp113\_fr\_001 &  32.41& -2.11 &  0.93 &  0.73&  St &   72.11 &  40.106 &  11.606 &    27.4 &   -40.9\\
189 bp120\_fr\_001 &   0.08& -3.67 &  0.84 &  0.73&  NSt &  169.48 &   4.930 &   1.018 &   119.6 &   -78.9\\
\hline
\end{longtable}
\end{center}

